StableQuant: Layer Adaptive Post-Training Quantization for Speech Foundation Models

In this paper, we propose StableQuant, a novel adaptive post-training quantization (PTQ) algorithm for widely used speech foundation models (SFMs). While PTQ has been successfully employed for compressing large language models (LLMs) due to its ability to bypass additional fine-tuning, directly applying these techniques to SFMs may not yield optimal results, as SFMs utilize distinct network architecture for feature extraction. StableQuant demonstrates optimal quantization performance regardless of the network architecture type, as it adaptively determines the quantization range for each layer by analyzing both the scale distributions and overall performance. We evaluate our algorithm on two SFMs, HuBERT and wav2vec2.0, for an automatic speech recognition (ASR) task, and achieve superior performance compared to traditional PTQ methods. StableQuant successfully reduces the sizes of SFM models to a quarter and doubles the inference speed while limiting the word error rate (WER) performance drop to less than 0.3% with 8-bit quantization.

==> 5_Results_1.tex <==
% Yeona : 이건 outlier 제거하지 않은 기존 방법의 mse 성능 결과



% 참고용: downstream layer quantize 안한것도 별 차이 없음!
% \begin{table}[t]
% \centering
% \caption{WER~(\%) results of base SFMs and downstream task models (will be removed at the end)}
% \vspace{5pt}
% \label{tab:comparison}
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|c|c}
% \Xhline{1pt}
% \textbf{Quant. types} & \textbf{HuBERT} & \textbf{wav2vec2.0} \\ \hline
% Base model & 3.06 & - \\
% All layers & 3.07 & 3.43 \\ \hline

% \Xhline{1pt}
% \end{tabular}
% % }
% \end{table}



\input{fig/inference_speed}


%\input{tables/calib_comparison}

%\input{fig/layer_out_distribution}

% \section{Results and Analysis}
% Kang: 4장과 5장을 합치는 것이 좋을 것 같음.

% Kang: 제목 수정 필요
% Woojin: 제안한 PTQ scheme이랑 다음 subsection의 removal이 같은 것 아닌가요?
% Yeona: 다릅니다. 제안한 scheme은 outlier removal 포함 percetile based의 MSE를 사용합니다.
\subsection{Comparison with traditional PTQ schemes}
% Kang: 혹시 quantization 이후에 적당한 speech data를 사용해서 SSL model을 fine-tuning한 후에 (QAT), 지금까지 PTQ로 얻은 성능과 비교해볼 수 있을까? 별 차이가 없다고 보여줄 수 있으면 매우 좋을 것 같은데. (시간이 부족하면 data를 많이 사용하지 않고 fine-tuning해보는 것도 괜찮음. 이를 통해서 data가 많지 않으면 fine-tuning하는 것이 효과없다는 형태로 서술할 수 있으므로)
% yeaon: qat 진행중입니다
% hyewon: 우선 위에 한 줄정도 언급하긴했는데 결과를 다시 확인해보아야합니다.
% PTQ의 장점
% 1. Table 3 에서 보다시피 base 모델보다 성능이 좋음. 즉 추가적인 트레이닝 없이도 큰 모델의 특성을 유지한채 줄임으로서 효율적인 모델 활용이 가능.
% QAT는 결과를 더 지켜봐야함. 분량 생각해보면 더 넣는게 맞을까요?
% 2. Activation을 quantize 했을 때 
To evaluate the effectiveness of our PTQ approach, we compared the performance of the proposed quantized ASR model to baseline models using various criteria, including word error rate (WER), inference speed, and model size. Table~\ref{tab:comparison} and Figure~\ref{fig:speed} summarize the results based on the quantization precision of weights and activations, respectively.


% 속도에 대한 gain -> activation quantization의 중요성
% \vspace{-5pt}
As the length of the speech to be processed increases, models quantized using our method obtain more significant gains in inference speed.
Moreover, quantizing activation values yields greater improvements in inference speed compared to quantizing weights at the same precision. This indicates that activation values significantly impact inference speed while quantizing weights primarily contributes to reducing model size.
% 여기서는 Table 3에 대한 장점 설명
As shown in Table~\ref{tab:comparison}, applying \shortname~in 8-bits dramatically compresses HuBERT-Large down to the same size as HuBERT-Base at full precision (32 bits) while achieving superior performance.
Moreover, it surpasses the quantization-aware training~(QAT) scheme~\cite{gholami2022survey} on \texttt{train-clean-100}.
This demonstrates that employing a carefully designed quantization scheme can be highly beneficial for speeding up existing large models compared to separately training smaller models, thus yielding time- and cost-efficient results.

% 여기 다시써야됨 (저번주에 결과 예상하고 쓴 부분이라..)
% 수정된 결과 바탕으로 다시 쓰긴했는데 표현 다듬기 필요함
\subsection{Effectiveness of \shortname}
Tabel.~\ref{tab:naive_quant} indicates the quantized results of activations comparing the transformer layers only and quantizing all layers including feature extractors with the existing MSE calibration method.
Quantizing the feature extraction layer results in significant performance drops than quantizing the Transformer layers at the same precision.
We hypothesize that this is due to the noisy distribution of activations in the feature extractors, as described in Sec.~\ref{sec:distribution}.
Moreover, wav2vec2.0 exhibits greater sensitivity than HuBERT.
This is a consistent result in Fig.~\ref{fig:distribution}(b), which implies that wav2vec2.0 exhibits broad distribution with larger variances, making it more prone to outliers.

As shown in Table.~\ref{tab:proposed}, removing outliers using percentiles before MSE during the scaling process for activations from selected layers leads to successful preservation of performance, even for 6-bits.
This achieves superior performance with quantized networks than applying existing approaches deployed independently.
From this result, a careful selection of scale factors by removing redundant outliers and informative criteria leads to stable preservation of information.





==> fig/layer_out_distribution.tex <==
% Yeona: quantized된 activation의 분포를 나타내려 했으나, 길다면 빼도 상관없을거 같음

\begin{figure}[t]
\begin{minipage}[t]{0.49\linewidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth] {fig/Analysis/wav2vec2_dist/hubert_0_1_seaborn_distribution.png}}
  \centerline{(b)}
  \centering
  \centerline{\includegraphics[width=\columnwidth] {fig/Analysis/wav2vec2_dist/hubert_0_1_seaborn_distribution.png}}
  \centerline{(d)}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\linewidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth] {fig/Analysis/wav2vec2_dist/hubert_0_1_seaborn_distribution.png}}
  \centerline{(b)}
  \centering
  \centerline{\includegraphics[width=\columnwidth] {fig/Analysis/wav2vec2_dist/hubert_0_1_seaborn_distribution.png}}
  \centerline{(d)}
\end{minipage}
\caption{Distribution of intermediate layer outputs. (a)-(b) denotes from x-th convolution layer outputs of HuBERT.}
\label{fig:distribution}
\end{figure}

==> fig/overall-workflow.tex <==
\begin{figure*}[h!]
\centering
% \includegraphics[width=0.8\textwidth]{fig/Analysis/archi/overall-workflow.png}
\includegraphics[width=0.85\textwidth]{fig/Analysis/archi/stable_quant_architecture.png}
\vspace{-10pt}
\caption{Overall workflow of StableQuant}
\label{fig:overallworkflow}
\end{figure*}
\vspace{-10pt}


==> fig/rebuttal_architecture.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=.95\columnwidth]{fig/Analysis/archi/overall-workflow-inter.png}
\caption{Overall workflow of StableQuant}
% \vspace{-10pt}
% \vspace{-0.5cm}  % 본문과의 간격 줄임
\label{fig:overallworkflow}
\end{figure}





% \vspace{-5pt}
% \begin{figure}[!t]
% \onecolumn 
% \centering
% \includegraphics[width=1.\linewidth]{fig/Analysis/archi/overall-workflow.png}
% \caption{Overall workflow of StableQuant}
% \label{fig:overallworkflow}
% \end{figure}
% \twocolumn






==> tables/calib_comparison.tex <==
% log-scale로 고치기
\begin{figure}[t]
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
            width=12cm, % 그래프 너비
            height=8cm, % 그래프 높이
            xlabel={Percentile Ratios},
            ylabel={WER~(\%)(\downarrow)},
            xmin=99.9, xmax=100, % x축 범위
            %ymin=0, ymax=100, % y축 범위
            legend pos=north west, % 범례 위치
            legend style={draw=none, fill=none, font=\scriptsize, align=right},  % Remove border and fill
            grid=both, % 그리드 표시
            reverse x axis % x축 내림차순
        ]
        %\addplot[color=orange,mark=o] coordinates {
        %    (100,66.06) (99.9,66.06)
        %};
        %\addlegendentry{W6A6 MSE (wav2vec2.0)}

        % W8A8 Proposed (MSE+Percentile) (wav2vec2.0)
        \addplot[color=red,mark=o] coordinates {
            (100,5.18) (99.99,3.64) (99.97,3.45) 
            (99.96,3.40) (99.95,3.39) (99.94,3.12) (99.93,3.09)
            (99.92,3.09) (99.91,3.10) (99.90,3.12) (99.80,3.07)
        };
        \addlegendentry{W8A8 proposed (wav2vec2.0)}


        
        % W6A6 Proposed (MSE+Percentile) (wav2vec2.0)
        \addplot[color=green,mark=o] coordinates {
            (100,60.06) (99.99,26.17) (99.98,10.41) (99.97,9.24) 
            (99.96,8.72) (99.95,8.28) (99.94,7.80) (99.93,7.50)
            (99.92,7.32) (99.91,7.03) (99.90,6.86) (99.89,6.67)
            (99.88,6.48)
        };
        \addlegendentry{W6A6 proposed (wav2vec2.0)}
        
        % W4A4 MSE (wav2vec2.0)
        %\addplot[color=pink,mark=o] coordinates {
        %    (100,100) (99.8,99.24)
        %};

        % W4A8 MSE (wav2vec2.0)
        % \addplot[color=yellow,mark=o] coordinates {
        %    (100,34.03) (99.97, 22.07) (99.96, 21.73)
        % };
        % \addlegendentry{W4A8 Percentiled MSE (wav2vec2.0)}
        
        % W8A8 Proposed (MSE+Percentile) MSE (HuBERT)
        \addplot[color=cyan,mark=o] coordinates {
            (100,2.56) (99.98,2.77) (99.97,2.78) 
            (99.96,2.64) (99.95,2.54) (99.94,2.49) (99.93,2.47)
            (99.92,2.39) (99.91,2.37) (99.9,2.4) (99.8,2.35)
            (99.7,2.46)
        };
        \addlegendentry{W8A8 proposed (HuBERT)}


        
        
        % W6A6 Proposed (MSE+Percentile) MSE (HuBERT)
        \addplot[color=magenta,mark=o] coordinates {
            (100,6.33) (99.99,5.71) (99.98,6.26) (99.97,5.94) 
            (99.96,5.14) (99.95,4.88)
        };
        \addlegendentry{W6A6 proposed (HuBERT)}
        
        % W4A4 MSE (HuBERT)
        %\addplot[color=blue,mark=o] coordinates {
        %    (100,100) (99.8, 89.83)
        %};
        %\addlegendentry{W4A4 Percentiled MSE (HuBERT)}

\end{axis}
\end{tikzpicture}
\caption{Calibration Method Comparison }
\end{figure}

==> tables/rebuttal_comparison.tex <==
\begin{table}[h]
\centering
\caption{Comparison with conventional PTQ methods in terms of WERs~(\%) for HuBERT-Large model}
\vspace{-3pt}
\label{tab:rebut_comparison}
% \vspace{5pt}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{l||l|r}
% \Xhline{1pt}

% \toprule
%  \textbf{Model type} & \textbf{Precision} & \textbf{Model size} & \textbf{WER~(\%)} \\ \midrule
%  % HuBERT-Base~& W32A32 & 491 & 6.33 \\
%  HuBERT-Large~& W32A32 & 1205 & 2.16 \\ \midrule
%  MSE~& W8A8 & 353 & \textbf{2.56} \\
%  \textbf{StableQuant}~& W8A8 & \textbf{353} & \textbf{2.35} \\ 
%  %SmoothQuant~& W8A8 & \textbf{353} & \textbf{2.35} \\ 

%  % QAT~(lr$=0.001$)& W8A8 & \textbf{357} & 4.10 \\ 
%  % QAT~(lr$=0.0001$)~& W8A8 & \textbf{357} & \textbf{2.24} \\ 
%  AdaRound~\cite{nagel2020up}~& W8A8 & - & 2.66 \\ 

%  % wav2vec2.0~& W32A32 & 1203 & 2.78 \\
%  % wav2vec2.0-Base~& W32A32 & 360 & 3.21 \\ 
%  % \textbf{StableQuant}~& W8A8 & 343 & \textbf{3.07} \\
%  % % QAT~(lr$=0.001$)& W8A8 & - & 6.99 \\ 
%  % % QAT~(lr$=0.0001$)~& W8A8 & - & 5.28 \\ 
%  % AdaRound~\cite{nagel2020up}~& W8A8 & - & 100 \\
 
%  \bottomrule

\toprule
 \textbf{Optimization} & \textbf{Precision}  & \textbf{WER~(\%)} \\ \midrule
 % HuBERT-Base~& W32A32 & 491 & 6.33 \\
 Full precision~& W32A32 &  2.16 \\ \midrule
 \textbf{StableQuant}~& W8A8  & \textbf{2.35} \\ 
 MSE~& W8A8 &  2.56 \\
 %SmoothQuant~& W8A8 & \textbf{353} & \textbf{2.35} \\ 

 % QAT~(lr$=0.001$)& W8A8 & \textbf{357} & 4.10 \\ 
 % QAT~(lr$=0.0001$)~& W8A8 & \textbf{357} & \textbf{2.24} \\ 
 AdaRound~\cite{nagel2020up}~& W8A8  & 2.66 \\ 

 % wav2vec2.0~& W32A32 & 1203 & 2.78 \\
 % wav2vec2.0-Base~& W32A32 & 360 & 3.21 \\ 
 % \textbf{StableQuant}~& W8A8 & 343 & \textbf{3.07} \\
 % % QAT~(lr$=0.001$)& W8A8 & - & 6.99 \\ 
 % % QAT~(lr$=0.0001$)~& W8A8 & - & 5.28 \\ 
 % AdaRound~\cite{nagel2020up}~& W8A8 & - & 100 \\
 
 \bottomrule









 
 %
 
% Woojin: w2v2 결과들로 바꾸기
% smoothquant 는 conv에 적용 안 된거면 빼기
% MSE:
% HuBERT-Large with QAT~& W8A8 & \textbf{357} & 4.19 \\ \bottomrule

 % wav2vec2.0-Large~& W32A32 & 1203 & 2.78 \\
 % wav2vec2.0-Base~& W32A32 & 360 & 3.21 \\
 % wav2vec2.0-Large with PTQ~& W8A8 & \textbf{343} & \textbf{3.07} \\ 
 % wav2vec2.0 with QAT~& W8A8 & 347 & 5.72 \\ \bottomrule
% MSE:
% wav2vec2.0 with QAT~& W8A8 & \textbf{347} & 7.99 \\ \bottomrule

%\Xhline{1pt}
\end{tabular}
}
 \vspace{-8pt}
\end{table}
